A Spectroscopic Orbit for Regulus

We present a radial velocity study of the rapidly rotating B-star Regulus that indicates the star is a single-lined spectroscopic binary. The orbital period (40.11 d) and probable semimajor axis (0.35 AU) are large enough that the system is not interacting at present. However, the mass function suggests that the secondary has a low mass (M_2 > 0.30 M_sun), and we argue that the companion may be a white dwarf. Such a star would be the remnant of a former mass donor that was the source of the large spin angular momentum of Regulus itself.

==> README <==
Dr. Chris Sneden, Letters Editor
THE ASTROPHYSICAL JOURNAL LETTERS
apjletters@letters.as.utexas.edu

Dear Chris, 

Many thanks for your efforts in finding a referee and for the report on 
our paper "A Spectroscopic Orbit for Regulus" by Gies et al. (ApJL #22909).
We appreciate the referee's speedy and careful review, and below we
outline the changes we made in response to the report. 

> This manuscript presents the discovery that Regulus is a spectroscopic
> binary with a period of about 40 days. Normally a simple spectroscopic
> orbital solution would not warrant publication as an ApJ Letter, but
> in this case the star is of special interest in that its very rapid
> rotation is difficult to explain given its present evolutionary
> status. The authors' results and their plausible conclusion that the
> companion is a white dwarf provide a natural explanation through a
> previous episode of mass and angular momentum transfer. Indirect
> evidence for such a white dwarf has been reported previously in the
> form of ultraviolet excess. In my opinion this justifies publication
> in ApJL. The paper is fairly straightforward, concise, and very well
> written, and I have only a few corrections, comments, and
> suggestions the authors may wish to consider:

> * The correct HIP number is 49669.

Corrected. 

> * My own orbital solution based on the authors' data gives slightly
> different results for the orbital elements and derived quantities.
> Although this difference is not terribly important for this paper, it
> was a bit unexpected for such a straightforward problem. Perhaps the
> authors could double-check their results. Fixing the orbital period to
> 40.11 days and assuming a circular orbit, as the authors have done, I
> get the following using my codes:
>
> Gamma = +4.90 +/- 0.20 km/s
> K = 7.03 +/- 0.29 km/s
> T = 2,444,527.02 +/- 0.27 (HJD)
> asini = 5.58 +/- 0.23 R_Sun
> f(M) = 0.00144 +/- 0.00018 M_Sun
> 
> in which I have weighted the observations as the authors claim to have
> done.  Perhaps the disagreement has to do with differences in the
> methodology (I used Levenberg-Marquardt optimization)...

We are grateful that the referee made an independent assessment of 
the orbital solution.  The difference in the results is a consequence 
of a slightly different weighting scheme that was not fully given 
in the first version of the paper.  We revised Section 3, paragraph 1, 
line 10 as follows:
"Each measurement was assigned a weight proportional to the 
inverse square of the larger of the measurement error 
or 1~km~s$^{-1}$ (to account for possible systematic 
errors between results from different groups of observations).
Trials with other weighting schemes gave similar results."

> * The authors have fixed the period in their solution to the value
> determined with the DFT and CLEAN methods. Given that the observations
> cover more than 250 cycles, I tried leaving P as a free parameter, and
> got a seemingly more precise value of 40.1160 +/- 0.0096 days (a
> factor of two better than reported in the manuscript). The change in
> the other elements is insignificant, except that the nodal passage
> becomes formally more poorly determined (2,444,525.9 +/- 1.9 days),
> although this is only because of the very strong correlation between P
> and T (with a correlation coefficient of -0.9899). Holding the period
> fixed, as the authors have done, artificially suppresses this
> correlation so that the nodal passage looks more precise but doesn't
> account for the error in P.

Again, the different (lower) error estimate for the period is due
to differences in the weighting scheme.  The referee used the inverse 
square of the quoted errors while we adopted the nominal equal weights 
used in the DFT/CLEAN method.  We prefer to adopt the more conservative 
errors associated with the standard time series analysis.  

We agree with the referee that the formal error for epoch does not 
account for the error in period (set to a constant in the orbital fit).  
We added to Section 3, paragraph 1, line 13 the following:
"Note that the error in $T_0$ increases to $\pm 3.9$~d
when the full range in acceptable period is considered."

> * In Sect. 4 the authors comment on the lack of evidence for the
> companion in observations that should have resolved it. It would be
> useful to include a few references here for those negative attempts.

We added citations to the interferometric and lunar occultation 
work on Regulus that failed to find evidence of a companion. 

> * In Table 3, it would be useful to include the estimate of the
> coefficient in the expression for M*sini, along with its error.

We added a new row to Table 3 with this functional parameter. 


We hope you will now find the paper ready for publication in the
Astrophysical Journal Letters. 

Sincerely yours, 

Douglas Gies

